A Comparative Analysis of Knowledge-Intensive and Data-Intensive Semantic Parsers

We present a phenomenon-oriented comparative analysis of the two dominant approaches in task-independent semantic parsing: classic, knowledge-intensive and neural, data-intensive models. To reflect state-of-the-art neural NLP technologies, we introduce a new target structure-centric parser that can produce semantic graphs much more accurately than previous data-driven parsers. We then show that, in spite of comparable performance overall, knowledge- and data-intensive models produce different types of errors, in a way that can be explained by their theoretical properties. This analysis leads to new directions for parser development.

==> tikzed-graphs/eds_example_complicate.tex <==
% \documentclass{article}
% \usepackage[x11names, rgb]{xcolor}
% \usepackage[utf8]{inputenc}
% \usepackage{tikz}
% \usetikzlibrary{snakes,arrows,shapes}
% \usepackage{amsmath}
% %
%

%


%
%
%

% \enlargethispage{100cm}
% Start of code
% \begin{tikzpicture}[anchor=mid,>=latex',line join=bevel,]
\begin{tikzpicture}[>=latex',line join=bevel,]
  \pgfsetlinewidth{1bp}
%%
\pgfsetcolor{black}

  % Node: e3
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \node(e3name) at (87.5bp,240.8bp) {{\texttt{\_manage\_v\_1}}} ;
  \node(e3) at (87.5bp,225.8bp) {\texttt{<1:2>}};
\end{scope}

  % Edge: _1 -> x5
  \draw [->] (60.866bp,106.28bp) .. controls (67.64bp,95.189bp) and (76.26bp,82.404bp)  .. (85.5bp,72.0bp) .. controls (90.856bp,65.969bp) and (97.046bp,60.053bp)  .. (111.15bp,47.95bp);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (96.5bp,79.5bp) node {BV};
  % Edge: e14 -> e16
  \draw [->] (315.59bp,230.2bp) .. controls (357.01bp,222.92bp) and (413.98bp,209.95bp)  .. (427.5bp,192.0bp) .. controls (436.38bp,180.21bp) and (429.07bp,168.38bp)  .. (408.89bp,152.41bp);
  \draw (461.5bp,184.5bp) node {R-HNDL};
  % Edge: e14 -> e16
  \draw [->] (299.45bp,215.68bp) .. controls (308.25bp,208.6bp) and (317.65bp,200.37bp)  .. (325.5bp,192.0bp) .. controls (332.73bp,184.29bp) and (339.77bp,175.32bp)  .. (351.91bp,158.25bp);
  \draw (371.0bp,184.5bp) node {R-INDEX};
  % Edge: e16 -> x5
  \draw [->] (338.09bp,108.35bp) .. controls (321.47bp,96.255bp) and (300.12bp,82.013bp)  .. (279.5bp,72.0bp) .. controls (251.27bp,58.293bp) and (217.88bp,47.375bp)  .. (181.11bp,37.059bp);
  \draw (326.5bp,79.5bp) node {ARG1};
  % Edge: e11 -> x5
  \draw [->] (187.45bp,108.0bp) .. controls (180.31bp,101.69bp) and (173.19bp,94.525bp)  .. (167.5bp,87.0bp) .. controls (161.96bp,79.67bp) and (157.15bp,71.069bp)  .. (149.0bp,53.442bp);
  \draw (188.5bp,79.5bp) node {ARG1};
  % Edge: x2 -> x12
  \draw [->] (466.99bp,109.73bp) .. controls (448.9bp,94.533bp) and (424.7bp,74.205bp)  .. (397.15bp,51.064bp);
  \draw (448.5bp,79.5bp) node {BV};
  % Edge: e3 -> x5
  \path [->] (e3) edge node [below] {ARG1}  (139.31bp,54.098bp);

%   \draw (159.5bp,184.5bp) node {ARG1};
  % Edge: e16 -> x12
  \draw [->] (368.5bp,104.96bp) .. controls (368.5bp,92.686bp) and (368.5bp,77.962bp)  .. (368.5bp,54.313bp);
  \draw (389.5bp,79.5bp) node {ARG2};
  % Edge: e14 -> e11
  \draw [->] (228.87bp,224.71bp) .. controls (213.04bp,217.79bp) and (196.64bp,207.35bp)  .. (187.5bp,192.0bp) .. controls (182.52bp,183.64bp) and (184.07bp,174.45bp)  .. (193.88bp,157.1bp);
  \draw (218.0bp,184.5bp) node {L-HNDL};
  % Edge: e14 -> e11
  \draw [->] (262.09bp,210.19bp) .. controls (258.41bp,199.62bp) and (253.74bp,187.53bp)  .. (248.5bp,177.0bp) .. controls (246.83bp,173.64bp) and (244.96bp,170.22bp)  .. (237.68bp,158.08bp);
  \draw (288.5bp,184.5bp) node {L-INDEX};
  % Edge: e11 -> x12
  \draw [->] (222.17bp,104.74bp) .. controls (224.56bp,93.363bp) and (229.06bp,80.781bp)  .. (237.5bp,72.0bp) .. controls (253.76bp,55.087bp) and (276.65bp,44.529bp)  .. (308.5bp,35.266bp);
  \draw (258.5bp,79.5bp) node {ARG2};
  % Edge: e3 -> e14
   \path [->] (e3) edge node [below] {ARG2}  (242.82bp,238.86bp);
%   \draw [->] (169.02bp,317.12bp) .. controls (188.82bp,301.48bp) and (214.41bp,281.28bp)  .. (242.82bp,258.86bp);
%   \draw (233.5bp,289.5bp) node {ARG2};
  % Node: e11
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (219.5bp,135.8bp) node {\texttt{\_house\_v\_1}};
  \draw (219.5bp,120.8bp) node {\texttt{<3:4>}};
\end{scope}
  % Node: e14
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (270.5bp,240.8bp) node {\texttt{\_and\_c}};
  \draw (270.5bp,225.8bp) node {\texttt{<4:5>}};
\end{scope}
  % Node: _1
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (46.5bp,135.8bp) node {\texttt{pron\_q}};
  \draw (46.5bp,120.8bp) node {\texttt{<0:1>}};
\end{scope}
  % Node: e16
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (368.5bp,135.8bp) node {\texttt{\_feed\_v\_1}};
  \draw (368.5bp,120.8bp) node {\texttt{<5:6>}};
\end{scope}
  % Node: x2
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (493.5bp,135.8bp) node {\texttt{\_the\_q}};
  \draw (493.5bp,120.8bp) node {\texttt{<6:7>}};
\end{scope}
  % Node: x12
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (368.5bp,30.8bp) node {\texttt{\_poor\_n\_1}};
  \draw (368.5bp,15.8bp) node {\texttt{<7:8>}};
\end{scope}

  % Node: x5
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (139.5bp,30.8bp) node {\texttt{pron}};
  \draw (139.5bp,15.8bp) node {\texttt{<0:1>}};
\end{scope}
%
\end{tikzpicture}
% End of code

%





==> tikzed-graphs/eds_example_map.tex <==
\begin{tikzpicture}[>=latex',line join=bevel,]
  \pgfsetlinewidth{1bp}
%%
\pgfsetcolor{black}
  % Edge: 5 -> 6
  \draw [->] (318.34bp,219.98bp) .. controls (334.2bp,211.93bp) and (353.05bp,201.92bp)  .. (369.5bp,192.0bp) .. controls (386.18bp,181.94bp) and (403.99bp,169.9bp)  .. (427.69bp,153.18bp);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (413.5bp,184.5bp) node {ARG2};
  % Edge: 7 -> 6
  \draw [->] (436.45bp,209.96bp) .. controls (439.67bp,197.47bp) and (443.53bp,182.44bp)  .. (449.57bp,158.95bp);
  \draw (456.5bp,184.5bp) node {BV};
  % Edge: 13 -> 12
  \draw [->] (710.01bp,210.23bp) .. controls (704.02bp,197.4bp) and (696.76bp,181.84bp)  .. (685.97bp,158.72bp);
  \draw (711.5bp,184.5bp) node {BV};
  % Edge: 5 -> 4
  \draw [->] (269.06bp,211.03bp) .. controls (266.35bp,204.96bp) and (263.92bp,198.4bp)  .. (262.5bp,192.0bp) .. controls (260.81bp,184.4bp) and (261.48bp,176.35bp)  .. (266.3bp,158.96bp);
  \draw (283.5bp,184.5bp) node {ARG1};
  % Edge: 8 -> 9
  \draw [->] (944.06bp,211.31bp) .. controls (962.94bp,195.95bp) and (986.97bp,176.39bp)  .. (1014.2bp,154.22bp);
  \draw (1005.5bp,184.5bp) node {ARG2};
  % Edge: 10 -> 9
  \draw [->] (1073.5bp,210.23bp) .. controls (1068.2bp,197.3bp) and (1061.8bp,181.6bp)  .. (1052.3bp,158.36bp);
  \draw (1076.5bp,184.5bp) node {BV};
  % Edge: 3 -> 2
  \draw [->] (145.48bp,210.06bp) .. controls (142.35bp,195.09bp) and (138.72bp,176.09bp)  .. (136.5bp,159.0bp) .. controls (132.36bp,127.13bp) and (130.06bp,90.66bp)  .. (128.38bp,54.145bp);
  \draw (157.5bp,132.0bp) node {ARG2};
  % Edge: 11 -> 4
  \draw [->] (522.72bp,218.21bp) .. controls (513.83bp,215.05bp) and (504.47bp,212.11bp)  .. (495.5bp,210.0bp) .. controls (458.09bp,201.18bp) and (356.72bp,211.32bp)  .. (323.5bp,192.0bp) .. controls (313.49bp,186.18bp) and (305.19bp,177.0bp)  .. (293.12bp,158.88bp);
  \draw (344.5bp,184.5bp) node {ARG1};
  % Edge: 1 -> 2
  \draw [->] (64.409bp,107.1bp) .. controls (72.675bp,96.274bp) and (82.516bp,83.47bp)  .. (91.5bp,72.0bp) .. controls (94.43bp,68.259bp) and (97.513bp,64.356bp)  .. (106.85bp,52.628bp);
  \draw (102.5bp,79.5bp) node {BV};
  % Edge: 8 -> 6
  \draw [->] (844.16bp,217.74bp) .. controls (831.71bp,214.76bp) and (818.77bp,212.01bp)  .. (806.5bp,210.0bp) .. controls (701.82bp,192.84bp) and (670.34bp,221.69bp)  .. (568.5bp,192.0bp) .. controls (542.74bp,184.49bp) and (516.18bp,170.57bp)  .. (486.85bp,152.77bp);
  \draw (589.5bp,184.5bp) node {ARG1};
  % Edge: 11 -> 12
  \draw [->] (592.62bp,212.12bp) .. controls (607.04bp,197.84bp) and (625.3bp,179.75bp)  .. (648.19bp,157.07bp);
  \draw (648.5bp,184.5bp) node {ARG2};
  % Edge: 3 -> 4
  \draw [->] (175.2bp,213.7bp) .. controls (187.23bp,202.25bp) and (202.28bp,188.48bp)  .. (216.5bp,177.0bp) .. controls (222.31bp,172.31bp) and (228.58bp,167.55bp)  .. (243.33bp,156.89bp);
  \draw (237.5bp,184.5bp) node {ARG1};
  % Edge: 4 -> 2
  \draw [->] (244.24bp,107.12bp) .. controls (221.81bp,91.723bp) and (192.93bp,71.902bp)  .. (161.14bp,50.088bp);
  \draw (234.5bp,79.5bp) node {ARG2};
  % Node: 11
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (456.5bp,50.8bp) node {\color{orange} loc\_nonsp};
  \draw (456.5bp,35.8bp) node {<7:9>};
\end{scope}
  % Node: 10
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (1084.5bp,240.8bp) node {proper\_q};
  \draw (1084.5bp,225.8bp) node {<5:6>};
\end{scope}
  % Node: 13
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (722.5bp,240.8bp) node {\_this\_q\_dem};
  \draw (722.5bp,225.8bp) node {<7:8>};
\end{scope}
  % Node: 12
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (673.5bp,135.8bp) node {\color{orange} \_year\_n\_1};
  \draw (673.5bp,120.8bp) node {<8:9>};
\end{scope}
  % Node: 1
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (45.5bp,135.8bp) node {\_the\_q};
  \draw (45.5bp,120.8bp) node {<0:1>};
\end{scope}
  % Node: 3
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (151.5bp,240.8bp) node {\color{blue} parg\_d};
  \draw (151.5bp,225.8bp) node {<3:4>};
\end{scope}
  % Node: 2
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (127.5bp,30.8bp) node {\_drug\_n\_1};
  \draw (127.5bp,15.8bp) node {<1:2>};
\end{scope}
  % Node: 5
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (283.5bp,240.8bp) node {\_in\_p};
  \draw (283.5bp,225.8bp) node {<4:5>};
\end{scope}
  % Node: 4
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (280.5bp,135.8bp) node {\color{blue} \_introduce\_v\_to};
  \draw (280.5bp,120.8bp) node {<3:4>};
\end{scope}
  % Node: 7
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (429.5bp,240.8bp) node {proper\_q};
  \draw (429.5bp,225.8bp) node {<6:7>};
\end{scope}
  % Node: 6
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (456.5bp,135.8bp) node {named};
  \draw (456.5bp,120.8bp) node {<6:7>};
\end{scope}
  % Node: 9
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (1041.5bp,135.8bp) node {named};
  \draw (1041.5bp,120.8bp) node {<5:6>};
\end{scope}
  % Node: 8
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (912.5bp,240.8bp) node {compound\_name};
  \draw (912.5bp,225.8bp) node {<5:7>};
\end{scope}
%
\end{tikzpicture}

%\vspace{0.6cm}


==> tikzed-graphs/eds_example_map_old.tex <==
\begin{tikzpicture}[>=latex,line join=bevel,]
  \centering
  \pgfsetlinewidth{0.6bp}
  \pgfsetcolor{black}
  \begin{scope}
     
    \node (_the_q) at (44.0bp,-110.0bp) [draw,align=center,draw=none] {{\texttt{\_the\_q}} \\ {\texttt{<0:1>}}};   
    \node at (44.0bp,-96bp) [draw,draw = none] {\color{red} \texttt{1}}; 
    
    \node (_drug_n_1) at (110.0bp,-170.0bp) [draw,align=center,draw=none] {{\texttt{\_drug\_n\_1}} \\ {\texttt{<1:2>}}};    
    \node at (105.0bp,-156.0bp) [draw,draw = none] {\color{red} \texttt{2}}; 
    
    \node (parg_d) at (108.0bp,-45.0bp) [draw,align=center,draw=none] {{\texttt{{\color{blue} parg\_d}}} \\ {\texttt{<3:4>}}};    
    \node at (108.0bp,-31.0bp) [draw,draw = none] {\color{red} \texttt{3}}; 
    
    \node (_introduce_v_to) at (178.0bp,-110.0bp) [draw,align=center,draw=none] {{\texttt{ {\color{blue} \_introduce\_v\_to}}} \\ {\texttt{<3:4>}}};    
    \node at (178.0bp,-95bp) [draw,draw = none] {\color{red} \texttt{4}}; 
    
    \node (loc_nonsp) at (230.0bp,-170.0bp) [draw,align=center,draw=none] {{\texttt{{\color{orange} loc\_nonsp}}} \\ {\texttt{<7:9>}}};    
    \node at (230.0bp,-156.0bp) [draw,draw = none] {\color{red} \texttt{11}}; 
	
    \node (_in_p) at (220.0bp,-45.0bp) [draw,align=center,draw=none] {{\texttt{\_in\_p}} \\ {\texttt{<4:5>}}};    
    \node at (220.0bp,-31.0bp) [draw,draw = none] {\color{red} \texttt{5}}; 
	
    \node (named32) at (280.0bp,-110.0bp) [draw,align=center,draw=none] {{\texttt{named}} \\ {\texttt{<6:7>}}};    
     \node at (278.0bp,-96.0bp) [draw,draw = none] {\color{red} \texttt{6}}; 
    
    \node (proper_q32) at (290.0bp,-45.0bp) [draw,align=center,draw=none] {{\texttt{proper\_q}} \\ {\texttt{<6:7>}}};   
    \node at (290.0bp,-31.0bp) [draw,draw = none] {\color{red} \texttt{7}}; 
    
    \node (_year_n_1) at (350.0bp,-125.0bp) [draw,align=center,draw=none] {{\texttt{{\color{orange} \_year\_n\_1}}} \\ {\texttt{<8:9>}}};    
    \node at (350.0bp,-111.0bp) [draw,draw = none] {\color{red} \texttt{12}};

    \node (_this_q_dem) at (450.0bp,-170.0bp) [draw,align=center,draw=none] {{\texttt{\_this\_q\_dem}} \\ {\texttt{<7:8>}}};
    \node at (450.0bp,-156.0bp) [draw,draw = none] {\color{red} \texttt{13}};
    
    \node (named27) at (420.0bp,-110.0bp) [draw,align=center,draw=none] {{\texttt{named}} \\ {\texttt{<5:6>}}};
    \node at (420.0bp,-96.0bp) [draw,draw = none] {\color{red} \texttt{9}};
    
    \node (proper_q27) at (460.0bp,-45.0bp) [draw,align=center,draw=none] {{\texttt{proper\_q}} \\ {\texttt{<5:6>}}};
    \node at (460.0bp,-31.0bp) [draw,draw = none] {\color{red} \texttt{10}};
    
    \node (compound_name) at (375.0bp,-45.0bp) [draw,align=center,draw=none] {\color{green} {\texttt{compound\_name}} \\ {\texttt{<5:7>}}};
    \node at (375.0bp,-31.0bp) [draw,draw = none] {\color{red} \texttt{8}};

    \path [->] (_the_q) edge [bend right=10] node [pos=0.4,below] {\small{BV}} (_drug_n_1);
    \path [->] (parg_d) edge node [below] {\small{ARG2}} (_drug_n_1);
    \path [->] (_introduce_v_to) edge [bend left=10] node [pos=0.3,below] {\small{ARG2}} (_drug_n_1);
    \path [->] (parg_d) edge [bend left=15] node [below] {\small{ARG1}} (_introduce_v_to);
    \path [->] (loc_nonsp) edge [bend left=10] node [pos=0.6,below] {\small{ARG1}} (_introduce_v_to);
    \path [->] (_in_p) edge node [pos=0.3,below] {\small{ARG1}} (_introduce_v_to);
    \path [->] (loc_nonsp) edge [bend left=10] node [pos=0.6,below] {\small{ARG2}} (_year_n_1);
    \path [->] (_this_q_dem) edge [bend right=10] node [below] {\small{BV}} (_year_n_1);
    \path [->] (_in_p) edge node [pos=0.3,below] {\small{ARG2}} (named32);
    \path [->] (proper_q32) edge [bend right=10] node [pos=0.3,below] {\small{BV}} (named32);
    \path [->] (proper_q27) edge node [pos=0.3,below] {\small{BV}} (named27);
    \path [->] (compound_name) edge [bend right=10] node [pos=0.3,below] {\small{ARG1}} (named32);
    \path [->] (compound_name) edge [bend left=15] node [pos=0.3,below] {\small{ARG2}} (named27);

  \end{scope}
  
\end{tikzpicture}

\vspace{0.6cm}

